Universal Compression of Power-Law Distributions

English words and the outputs of many other natural processes are well-known to follow a Zipf distribution. Yet this thoroughly-established property has never been shown to help compress or predict these important processes. We show that the expected redundancy of Zipf distributions of order $\alpha>1$ is roughly the $1/\alpha$ power of the expected redundancy of unrestricted distributions. Hence for these orders, Zipf distributions can be better compressed and predicted than was previously known. Unlike the expected case, we show that worst-case redundancy is roughly the same for Zipf and for unrestricted distributions. Hence Zipf distributions have significantly different worst-case and expected redundancies, making them the first natural distribution class shown to have such a difference.

==> implication.tex <==
\textbf{Implication for natural-language processing}
English words are well-known to follow a Zipf distribution,
hence our results imply that when viewed as \iid\ they can 
be better compressed and predicted.
In practice, English text is compressed and
predicted based on past memory, for a simple example,
the previous two-word bi-gram. Still the words following
each bi-gram could very well be Zipf distributed and
it would be interesting to see whether the results
we derived could be used in that context to improve
natural language processing tasks.

